TorchOpera: A Compound AI System for LLM Safety

We introduce TorchOpera, a compound AI system for enhancing the safety and quality of prompts and responses for Large Language Models. TorchOpera ensures that all user prompts are safe, contextually grounded, and effectively processed, while enhancing LLM responses to be relevant and high quality. TorchOpera utilizes the vector database for contextual grounding, rule-based wrappers for flexible modifications, and specialized mechanisms for detecting and adjusting unsafe or incorrect content. We also provide a view of the compound AI system to reduce the computational cost. Extensive experiments show that TorchOpera ensures the safety, reliability, and applicability of LLMs in real-world settings while maintaining the efficiency of LLM responses.

==> experiment.tex <==

\section{Experiments}\label{sec: exp}


\textbf{Experimental Setting. }
We use our self-developed model, Fox-1~\cite{fox}, as our base model for finetuning safety detection models. 
Safety Detector model is trained with 15 datasets, as follows: 
HEx-PHI~\cite{anonymous2024finetuning}, 
OpenAI~\cite{openai-data-paper}, 
Hotpot QA~\cite{yang2018hotpotqa}, 
Truthful QA~\cite{lin2021truthfulqa}, 
Awesome ChatGPT Prompts~\cite{awesome-chatgpt-prompts}, 
Jigsaw Unintended-Bias Data~\cite{jigsaw-unintended-bias-in-toxicity-classification}, 
GPT-Jailbreak~\cite{ChatGPT-Jailbreak-Prompts}, 
Jailbreak ~\cite{jailbreak-classification},
Personalization Prompt~\cite{filtered_personalization_prompt_response}, 
QA Chat Prompts~\cite{qa-chat-prompts}, 
ChatGPT Prompts~\cite{ChatGPT-prompts}, 
10k Prompts Ranked~\cite{10k_prompts_ranked}, 
Iterative Prompt~\cite{iterative-prompt-v1-iter1-20K},  and 
Instruction Following~\cite{instruction-following}. Hallucination detection model is trained with HaluEval dataset \cite{li2023halueval} dataset. 
Grounding experiments are conducted on the following datasets:
E-Commerce~\cite{e_commerce_dataset},
ChatDoctor~\cite{ChatDoctor-dataset},
PatientDoctorChat~\cite{patient-doctor-chat-data}. 
Evaluations  and model training experiments  are conducted on a server with 8 NVIDIA
H100 GPUs. 

% \textbf{Models. }
% \begin{itemize}
%     % \item microsoft/Phi-3-mini-4k-instruct
%     % \item openai-community/gpt2   (137M)

%     \item mistralai/Mistral-7B-Instruct-v0.2: 
%     % \item meta-llama/Meta-Llama-3-8B-Instruct
%     \item tiiuae/falcon-40b-instruct  
%     \item GPT4 API
% \end{itemize}

% =============

\begin{table}[ht]
\centering
\caption{Training Data for \goodname~Safety Detector}
\label{tab
}
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Dataset} & \textbf{Train} & \textbf{Validation} & \textbf{Test} \\ \midrule
HEx-PHI~\cite{anonymous2024finetuning} & 330 & 0 & 0 \\
OpenAI~\cite{openai-data-paper}& 160 & 1500 & 0 \\
Hotpot QA~\cite{yang2018hotpotqa} & 3000 & 2500 & 500 \\
Truthful QA~\cite{lin2021truthfulqa} & 500 & 100 & 100 \\
Awesome ChatGPT Prompts~\cite{awesome-chatgpt-prompts} & 0 & 150 & 0 \\
Jigsaw Unintended-Bias Data~\cite{jigsaw-unintended-bias-in-toxicity-classification} & 100000 & 2000 & 300 \\
GPT-Jailbreak~\cite{ChatGPT-Jailbreak-Prompts} & 0 & 78 & 0 \\
Jailbreak~\cite{jailbreak-classification} & 400 & 0 & 70 \\
Personalization Prompt~\cite{filtered_personalization_prompt_response} & 1000 & 800 & 200 \\
QA Chat Prompts~\cite{qa-chat-prompts} & 0 & 200 & 0 \\
ChatGPT Prompts~\cite{ChatGPT-prompts} & 350 & 0 & 0 \\
10k Prompts Ranked~\cite{10k_prompts_ranked} & 500 & 500 & 200 \\
Iterative Prompt~\cite{iterative-prompt-v1-iter1-20K} & 500 & 500 & 200 \\
Instruction Following~\cite{instruction-following} & 200 & 340 & 0 \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Evaluation of Safety Detector}

\textbf{Exp 1. Unsafe user inputs detection. }
We fine-tuned a model to detect undesired contents or safety risks in user inputs, such as toxicity, prompt injection, stereotypes, harassment, threats, obscenities, identity attacks, and violence. To mitigate the discrepancies between distributions of opensource data and real-world user queries, instead of training with several datasets, we crafted a training dataset by randomly selecting data from 15 public data sources and combining them.  
The datasets and the number of records involved in training, validation, and test phases are summarized in Table \ref{tab
}. We compare our approach with 
Detoxify-Roberta~\cite{Detoxify},
Detoxify-BERT~\cite{Detoxify},
Nvidia NeMo GuardRail~\cite{nemo}, 
OpenAI Moderate~\cite{openai-data-paper}, and 
PerspectiveAPI~\cite{perspective-api} in  Table~\ref{tab:toxicity detecion}. Results show that our model achieves comparable performance with OpenAI API. 
Overall, our model demonstrates robust performance across key metrics, indicates its effectiveness and reliability in real-world applications. 



\begin{table}[ht]
\centering
\caption{Unsafe Content Detection Comparison}
\label{tab:toxicity detecion}
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Model} & \textbf{Accuracy} & \textbf{Recall} & \textbf{F1} \\ \midrule
Detoxify-Roberta~\cite{Detoxify} & 0.847 & 0.504 & 0.483 \\
Detoxify-BERT~\cite{Detoxify} & 0.872 & 0.568 & 0.585 \\
NeMo & 0.687 & 0.767 & 0.611 \\
OpenAI Moderate~\cite{openai-data-paper} & 0.878 & 0.573 & 0.595 \\
PerspectiveAPI~\cite{perspective-api} & 0.875 & 0.573 & 0.594 \\
Ours & 0.877 & 0.624 & 0.656 \\
\bottomrule
\end{tabular}
\end{table}


\textbf{Exp 2. Hallucination detection in LLM outputs. } 
We fine-tuned our hallucination detection model using the HaluEval dataset \cite{li2023halueval}. We utilized 8,000 data samples for training, 1,500 for validation, and 500 for testing. The fine-tuning process involved creating structured prompts that guided the model to identify hallucinations in the LLM outputs effectively.
Each data sample was formatted to include a system prompt, a user question, relevant contextual information, and an LLM-generated answer. An example of a processed training data entry is as follows:


% \textit{<INST> <<SYS>> You are a helpful assistant. <</SYS>> According to the Question and the Contexts, is there any hallucination in the LLM Answer?}

% Question: Which magazine was published first, Who Put the Bomp or Curve? \\
% Context: Who Put The Bomp was a rock music fanzine edited and published by Greg Shaw from 1970 to 1979. Its name came from the hit 1961 doo-wop song by Barry Mann, "Who Put the Bomp". It covers news, politics, social issues, and includes celebrity interviews and stories on entertainment, pop culture, style, travel, and a website that hosts an internet forum focusing on lesbian issues, active since 2000. \\
% LLM Answer: Curve was published before Who Put the Bomp. \\
% \#\#\# Response:</INST> Yes, the answer cannot be deduced from the context or the answer is useless.}

% <s>[INST] <<SYS>> You are a helpful assistant. <</SYS>> According to the Question and the Contexts, is there any hallucination in the LLM Answer?  Question: Which magazine was published first, Who Put the Bomp or Curve?; Context: Who Put The Bomp was a rock music fanzine edited and published by Greg Shaw from 1970 to 1979. Its name came from the hit 1961 doo-wop song by Barry Mann, "Who Put the Bomp". It covers news, politics, social issues, and includes celebrity interviews and stories on entertainment, pop culture, style, travel, and a website that hosts an internet forum focusing on lesbian issues, active since 2000.; LLM Answer: Curve was published before Who Put the Bomp.. ### Response:[/INST] Yes, the answer cannot be deduced from the context or the answer is useless.

\begin{quote}

\ttfamily
<INST> <<SYS>> You are a helpful assistant. <</SYS>> \\ According to the Question and the Contexts, is there any hallucination in the LLM Answer?

Question: Which magazine was published first, Who Put the Bomp or Curve? \\
Context: Who Put The Bomp was a rock music fanzine edited and published by Greg Shaw from 1970 to 1979. Its name came from the hit 1961 doo-wop song by Barry Mann, "Who Put the Bomp". It covers news, politics, social issues, and includes celebrity interviews and stories on entertainment, pop culture, style, travel, and a website that hosts an internet forum focusing on lesbian issues, active since 2000. \\
LLM Answer: Curve was published before Who Put the Bomp. \\
\#\#\# Response:</INST> Yes, the answer cannot be deduced from the context or the answer is useless.
\end{quote}


This structured format ensured that the model received a clear and consistent input while highlighting the context information as well as the instruction for the  hallucinations task. 
Our model achieved an accuracy of 0.928 on the testing dataset. 

% \begin{Verbatim}[frame=single]
% <INST> <<SYS>> You are a helpful assistant. <</SYS>> According to the Question and the Contexts, is there any hallucination in the LLM Answer?

% Question: Which magazine was published first, Who Put the Bomp or Curve?
% Context: Who Put The Bomp was a rock music fanzine edited and published by Greg Shaw from 1970 to 1979. Its name came from the hit 1961 doo-wop song by Barry Mann, "Who Put the Bomp". It covers news, politics, social issues, and includes celebrity interviews and stories on entertainment, pop culture, style, travel, and a website that hosts an internet forum focusing on lesbian issues, active since 2000.
% LLM Answer: Curve was published before Who Put the Bomp.
% ### Response:</INST> Yes, the answer cannot be deduced from the context or the answer is useless.
% \end{Verbatim}

% 'eval_accuracy': 0.876669449081803, 'eval_precision': 0.7621311920268403, 'eval_recall': 0.6235832992594612, 'eval_f1': 0.6563309283986363, 'eval_roc_auc': 0.8319629276270956, 'eval_runtime': 44.4077, 'eval_samples_per_second': 107.909, 'eval_steps_per_second': 3.378, 'epoch': 16.0


\begin{table}[htbp]
\centering
\caption{Call-backs of Original Data Records in Top-$k$ Queries}
\label{tab:exp-query-call-back}
\small
\begin{tabular}{@{}llcccccccc@{}}
\toprule
\textbf{Dataset} & \textbf{Query Type} & \multicolumn{4}{c}{\textbf{Whole Knowledge Indexing}} & \multicolumn{4}{c}{\textbf{Key Information Indexing}} \\ 
\cmidrule(lr){3-6} \cmidrule(l){7-10}
& & \textbf{Top1} & \textbf{Top3} & \textbf{Top5} & \textbf{Top10} & \textbf{Top1} & \textbf{Top3} & \textbf{Top5} & \textbf{Top10} \\
\midrule
\multirow{2}{*}{E-Commerce~\cite{e_commerce_dataset}} & Original & 0.96 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
                                                      & Rephrased & 0.82 & 1.00 & 1.00 & 1.00 & 0.92 & 0.98 & 1.00 & 1.00 \\
\addlinespace
\multirow{2}{*}{ChatDoctor~\cite{ChatDoctor-dataset}}                  & Original & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
                                                      & Rephrased & 0.66 & 0.78 & 0.80 & 0.82 & 0.88 & 0.94 & 0.96 & 0.98 \\
\addlinespace
\multirow{2}{*}{PatientDoctorChat~\cite{patient-doctor-chat-data}}          & Original & 0.72 & 0.90 & 0.96 & 0.98 & 0.96 & 1.00 & 1.00 & 1.00 \\
                                                      & Rephrased & 0.56 & 0.74 & 0.76 & 0.80 & 0.78 & 0.92 & 0.94 & 0.96 \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Evaluation of Grounding}
\textbf{Exp 3. Evaluation of callbacks for supplementary information retrieval. }
We evaluate the effectiveness of TensorOpera Grounding in retrieving complementary information from the vector data storage. This evaluation utilizes three QA datasets, including E-Commerce dataset~\cite{e_commerce_dataset} that contains customer service interactions on an online platform, and two healthcare datasets, Patient-Doctor Chat dataset~\cite{patient-doctor-chat-data} and the ChatDoctor dataset~\cite{ChatDoctor-dataset}, which contain QA pairs between doctors and patients. 
Precision in retrieving knowledge is critical in these scenarios, as inaccuracies can lead to financial losses and harmful medical advice.
To comprehensively evaluate retrieval performance and simulate user queries real-world applications, we used both original and rephrased queries. Original queries matched those questions in the datasets, while rephrased queries, generated by TinyLlama~\cite{zhang2024tinyllama} or a summarization model~\cite{summarization-model}, simulate variability in user questions. We measured the ``call-back rate'' (i.e., retrieval success rate) with Top-$k$ queries, where $k$ is set to 1, 3, 5, and 10. Retrieval was considered successful if the retrieved $k$ records contained the original records in the datasets. We recorded the call-back rates in Table~\ref{tab:exp-query-call-back}.
The results indicate that Key Information Indexing outperformed Whole Knowledge Indexing, as key information indexes reflects the user queries better. Also, both original queries and rephrased queries achieved high call-back rates, which demonstrates the effectiveness of vector retrieval when handling varied user inputs.


\begin{table}[ht]
\centering
\caption{URL Detection Task}
\label{tab:fixing_exp}
\small
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Metrics} & \textbf{Fixing (Ours)} & \textbf{TinyLLama} & \textbf{Mistral-7B} & \textbf{LLama2-7B} & \textbf{LLama3-8B} & \textbf{Falcon-40B} \\ \midrule
Avg. Time (s) & \textbf{1.06} & 13.17 & 10.93 & 9.10 & 20.10 & 34.67 \\
% Detected URL num & 24 & 0 & 22 & 20 & 9 & 0 \\
Detection Acc. & \textbf{100.00\%} & {\redxmark} {(Fail)} & 91.67\% & 83.33\% & 37.50\% & {\redxmark} {(Fail)} \\
Validation Acc. & \textbf{83.33\%} & {\redxmark} {(Fail)}& 45.83\% & 54.17\% & 37.50\% & {\redxmark} {Fail} \\
\bottomrule
\end{tabular}
\end{table}



\subsection{Evaluation of TorchOpera Repairer}
\textbf{Eexp 4. Efficiency of fixing. }
We evaluated the efficiency of TorchOpera Repairer in identifying and addressing problematic content in LLM outputs with the URL detection and validation task described in \S\ref{sec:fixing}. 
% The objective was to detect if LLM outputs contain URLs and prepend a warning message of the unsafe URLs at the beginning of the URLs. If URLs were found, the Fixing module should check their safety, i.e., whether they are malicious or unreachable, and including this information in the warning if they were unsafe.
We randomly select 15 records from the E-Commerce dataset~\cite{e_commerce_dataset} and the RedditSYACURL Dataset~\cite{reddit-url-data}, combine each record to construct texts that contain URLs, and set 20\% probability of inserting some malicious URLs into the text. In implementation, we use Regex pattern for detecting URLs, then utilize Google SafeBrowsing for detecting malicious URLs, and send HTTP requests to the unmalicious URLs to verify their reachability.
We compared TorchOpera Repairer with several models, including TinyLLama~\cite{zhang2024tinyllama}, Mistral-7B~\cite{jiang2023mistral}, LLama2-7B~\cite{touvron2023llama}, and Falcon-40B~\cite{falcon40b}. 
The results are shown in Table~\ref{tab:fixing_exp}. We record average time to process one query, the success rate of detecting URLs (Detection Acc.), and the accuracy of identifying unsafe URLs (Validation Acc.).
The results show that while TorchOpera Repairer takes much less time (1.06s per query), it
significantly outperforms calling the models for fixing LLM outputs. Also, TinyLLama and Falcon-40B failed to detect any URLs in the contents. Though Mistral is able to detect URLs with a high accuracy of 91.67\%, the accuracy of identifying unsafe URLs is only 45.83\%.




% 1. url detection wrapper vs 
% 2. (worse utility) prompt egineering: llm to extract urls and verify reachability / malicious
% 3. llm to extract urls + code for reachability + model for malicious url + put them together

% LLM generate text one by one, so has to detect after 

% our model (1B): \~ 159s for 15 queries; results are not good because we haven't do alignment

% one more wrapper example: substitution words; add suggested reading time; 


% \begin{table}[h!]
%   \centering
%   \small
%   \caption{Dataset Overview with Placeholder Metrics}
%   \begin{tabular}{lccccc}
%     \toprule
%     Dataset Name & Data Size & VectorDB Storage & (Ours) VectorDB Storage & AVG Searching Time & Call-back Rate \\
%     \midrule
%     Customer Service & 65 & - & - & - & - \\
%     News Summary & 21,417 & - & - & - & - \\
%     Chat Doctor & 119,486 & - & - & - & - \\
%     AI Medical Chatbot & 256,916 & - & - & - & - \\
%     Patient Doctor Chat & 379,460 & - & - & - & - \\
%     \bottomrule
%   \end{tabular}
%   \label{tab:dataset_metrics}
% \end{table}




% current rag splits long documents into truncks as they may want to search for detailed info. However, for real products, the knowledge can be short and focus on single topic; thus do not need to store all data






==> tables_and_algos/dataset_table.tex <==

\begin{table}[htbp]
\centering
\scriptsize
\caption{Dataset Descriptions}
\label{tab:datasets}
\begin{center}
\begin{tabular}{p{1.8cm}p{2.6cm}p{1.4cm}p{6cm}}
\toprule
\textbf{Task} & \textbf{Dataset} & \textbf{Data size} & \textbf{Description} \\
\midrule

\multirow{9}{8em}{\\Unsafe \\Content\\ Detection} & HEx-PHI~\cite{anonymous2024finetuning} & 330 & This dataset contains 330 harmful instructions (30 examples x 11 prohibited categories) for LLM harmfulness evaluation. 
\\\cline{2-4}
\addlinespace

 & OpenAI~\cite{openai-data-paper} & 1680 & OpenAI moderation dataset that contains prompts that are annotated with their own taxonomy. \\\cline{2-4}
\addlinespace
 & Hotpot QA~\cite{yang2018hotpotqa} & 113k & QA pairs based on Wikipedia knowledge. \\\cline{2-4}
\addlinespace
 & Truthful QA~\cite{lin2021truthfulqa} & 827 & A QA dataset that contains 817 questions spanning 38 categories, including health, law, finance, and politics. \\\cline{2-4}
\addlinespace
 & Awesome GPT Prompts~\cite{awesome-chatgpt-prompts} & 153 & Awesome prompt examples to be used with ChatGPT. \\\cline{2-4}
\addlinespace
 & Jigsaw Unintended-Bias Data~\cite{jigsaw-unintended-bias-in-toxicity-classification} & 2M & Comment data that contains labels for unsafe content. \\\cline{2-4}
\addlinespace
 & GPT-Jailbreak~\cite{ChatGPT-Jailbreak-Prompts} & 79 & ChatGPT jailbreak prompts. \\\cline{2-4}
\addlinespace
 & Jailbreak~\cite{jailbreak-classification} & 1.3k & A dataset that contains jailbreak prompts and benign prompts. \\\cline{2-4}
\addlinespace
 & Personalization Prompt~\cite{filtered_personalization_prompt_response} & 10.4k & Prompt-response pairs for personalized interactions with LLMs. \\\cline{2-4}
\addlinespace
 & QA-Chat Prompts~\cite{qa-chat-prompts} & 200 & A QA dataset. \\\cline{2-4}
\addlinespace
 & ChatGPT Prompts~\cite{ChatGPT-prompts} & 360 & A dataset that contains human prompts and ChatGPT responses. \\\cline{2-4}
\addlinespace
 & 10k-Prompts Ranked~\cite{10k_prompts_ranked} & 10.3k & A dataset of prompts with quality rankings created by 314 members of the open-source ML community using Argilla, an open-source tool to label data. \\\cline{2-4}
\addlinespace
 & Iterative Prompt~\cite{iterative-prompt-v1-iter1-20K} & 20k & A dataset of user prompts. \\\cline{2-4}
\addlinespace
 & Instruction Following~\cite{instruction-following} & 514 & An instruction dataset. \\
 \cline{2-4}
 \addlinespace
 & ToxicChat~\cite{lin2023toxicchat} & 10165 & [Evaluation data in \textbf{Exp1}] A dataset for toxicity detection.  \\\cline{2-4}
\hline
\\ Hallucination Detection & HaluEval~\cite{li2023halueval} & 10k & A dataset for evaluating hallucinations. We utilize the ``qa'' subset that contains dialogue histories, contexts (knowledge), right responses, and hallucinated responses. \\\cline{2-4}
\hline

\multirow{3}{8em}{Vector\\ Retrieval \\Evaluation} & E-Commerce~\cite{e_commerce_dataset} & 65 & We use the ``faq'' subset that contains QA pairs between users and service agents. \\\cline{2-4}
\addlinespace

  & Patient-Doctor Chat~\cite{patient-doctor-chat-data} & 379k & Dialogue data between doctors and patients. \\\cline{2-4}\addlinespace

  & ChatDoctor dataset~\cite{ChatDoctor-dataset} & 119.4 & Dialogue data between doctors and patients. \\
\hline
\multirow{2}{8em}{\\Repairere\\ Wrapper\\ Evaluation} & E-Commerce dataset~\cite{e_commerce_dataset} & 1.89k & We use the "faq" subset (as described above) and the "product" subset that contains descriptions of products. \\\cline{2-4}\addlinespace

 & RedditSYACURL Dataset~\cite{reddit-url-data} & 8.61k & A dataset that contains titles, summaries, and links of articles.\\ \bottomrule
\end{tabular}
\end{center}
\end{table}

==> tables_and_algos/hallucination_data_processing_algo.tex <==


\LinesNotNumbered \begin{algorithm}[!t]
\textbf{Inputs:} \\
$\mathcal{D}$: a training dataset that contains ``context'' (knowledge), ``inputs'', ``llm\_answer'', and ``labels'' for hallucination.  
%$R$: a relation. $\mathbb{H}$: A hash function. $\mathcal{E}()$: An encryption function. $s_k$: a secret key.

\textbf{Outputs:} $\mathcal{D}_t$: the training dataset.

\textbf{Variables:} \\
\textit{response\_template}: ``{\#\#\# Response:}''; \\

\textit{\text{prompt}\_\text{template}}: ``{<s>[INST] <<SYS>> You are a helpful assistant. 
<</SYS>> According to the} \\

{~~Question and the Context, is there any hallucination in the Answer? Question: \{\textbf{question}\};} \\ {~~Context: \{\textbf{context}\}; LLM Answer: \{\textbf{llm\_answer}\}. 
\{\textit{response}\_\textit{template}\}[/INST] \{\textbf{response}\}. }''\\

\textit{GPT\_reasoning\_template}: ``
{Explain why there is hallucination in the LLM answer. Question:}\\ {~~\{\textbf{question}\}; Context: \{\textbf{context}\}; LLM Answer: \{\textbf{llm\_answer}\}.}
''



\nl{\bf Function $\boldsymbol{\mathit{process\_data}(\mathcal{D})}$} \nllabel{ln:function_process_data}
\Begin{

\nl $\mathcal{D}_t\leftarrow \phi$

\nl \For{$d \in \mathcal{D}$}{

\nl \eIf{$\mathit{is}\_\mathit{hallucination}$($d$)}{

\nl $\mathit{hallucination}\_\mathit{reason}\leftarrow\mathit{GPT}\_\mathit{API}$(\textit{GPT}\_\textit{reasoning}\_\textit{template}($d$[`$\mathit{question}$'], $d$[`$\mathit{context}$'], $d$[`$\mathit{llm}\_\mathit{answer}$']))

\nl $\mathit{response}\leftarrow$ ``Yes, '' + $\mathit{hallucination}\_\mathit{reason}$


\nl $d^\prime\leftarrow$\textit{prompt}\_\textit{template}($d$[`$\mathit{question}$'], $d$[`$\mathit{context}$'], $d$[`$\mathit{llm}\_\mathit{answer}$'], $\mathit{response}$)

}{

\nl $d^\prime\leftarrow$\textit{prompt}\_\textit{template}($d$[`$\mathit{question}$'], $d$[`$\mathit{context}$'], $d$[`$\mathit{llm}\_\mathit{answer}$'], ``$\mathit{No.}$'')


}

\nl $\mathcal{D}_t\leftarrow d^\prime$

}

\nl \textbf{return $\mathcal{D}_t$}
}

\caption{Training data processing for hallucination detection.}
\label{alg:hallucination_data_processing}
\end{algorithm}


==> tables_and_algos/hallucination_inference_algo.tex <==


\LinesNotNumbered \begin{algorithm}[!t]
\textbf{Inputs:} 

$\mathcal{M}$: hallucination detection model.

$\mathit{tokenizer}$: tokenizer for $\mathcal{M}$.

$\mathit{question}$: a query submitted by users.

$\mathit{context}$: the context to answer the question; retrieved from vector data storage.

$\mathit{llm}\_\mathit{answer}$: the answer returned by an LLM for the question.  

% \textbf{Outputs:} $\mathcal{D}^\prime$: a processed dataset.

\textbf{Variables:} \\
\textit{response}\_\textit{template}: ``{\#\#\# Response:}''; \\

\textit{inference}\_\textit{prompt}\_\textit{template}: ``{<s>[INST] <<SYS>> You are a helpful assistant. 
<</SYS>>
According}\\ 
{~~to the Question and the Contexts, is there any hallucination in the LLM Answer?} Question: \\
{~~\{\textbf{question}\}; Context: \{\textbf{context}\}; LLM Answer: \{\textbf{llm\_answer}\}. \{{response}\_\textit{template}\}[/INST]}''\\

% \textit{GPT}\_\textit{reasoning}\_\textit{template} = ``
% Explain why there is hallucination in the LLM answer. Question: \{\textbf{question}\}; Context: \{\textbf{context}\}; LLM Answer: \{\textbf{llm\_answer}\}.
% ''



\nl{\bf Function $\boldsymbol{\mathit{inference}(\mathcal{M}, \mathit{question}, \mathit{context}, \mathit{llm\_answer})}$} \nllabel{ln:inference}
\Begin{


\nl $\mathit{prompt}\leftarrow$\textit{inference}\_\textit{prompt}\_\textit{template}($\mathit{question}$, $\mathit{context}$, $\mathit{llm}\_\mathit{answer}$)

\nl $\mathit{tokenized}\_\mathit{prompt}\leftarrow \mathit{tokenizer}$($\mathit{prompt}$), $\mathit{output}\leftarrow \mathcal{M}$.$\mathit{generate}$($\mathit{tokenized}\_\mathit{prompt}$)

\nl $\mathit{first}\_\mathit{word}\_\mathit{logits}\leftarrow \mathit{output}$.$\mathit{logits}$[0], $\mathit{probabilities}\leftarrow\mathit{softmax}$($\mathit{first}\_\mathit{word}\_\mathit{logits}$)

\nl $\mathit{top\_probs}$, $\mathit{top\_indices}\leftarrow \mathit{top10}$($\mathit{probabilities}$)

\nl $\mathit{yes}\_\mathit{prob}\leftarrow 0$, $\mathit{no}\_\mathit{prob}\leftarrow 0$

\nl \For{$i\in \mathit{range}$($\mathit{len}$($\mathit{top\_indices}$))}{

\nl $\mathit{first}\_\mathit{word}\leftarrow \mathit{tokenizer}$.$\mathit{decode}$($\mathit{top\_indices}$[$i$])

\nl \If{$\mathit{first}\_\mathit{word}\in$ [``Yes'', ``yes''] }{

$\mathit{yes}\_\mathit{prob}\leftarrow \mathit{yes}\_\mathit{prob} + \mathit{top\_probs}$[$i$]

}

\nl \If{$\mathit{first}\_\mathit{word}\in$ [``No'', ``no''] }{

$\mathit{no}\_\mathit{prob}\leftarrow \mathit{no}\_\mathit{prob} + \mathit{top\_probs}$[$i$]

}

}

\nl $\mathit{yes}\_\mathit{prob}\leftarrow \frac{\mathit{yes}\_\mathit{prob}}{\mathit{yes}\_\mathit{prob} + \mathit{no}\_\mathit{prob}}$, $\mathit{no}\_\mathit{prob}\leftarrow 1-\mathit{yes}\_\mathit{prob}$

\nl \eIf{$\mathit{yes}\_\mathit{prob}\geq \mathit{no}\_\mathit{prob}$}{\textbf{return} True}{\textbf{return} False}
}

\caption{Inference with hallucination detection model.}
\label{alg:inference}
\end{algorithm}
